Weakly-Supervised Methods for Suicide Risk Assessment: Role of Related Domains

Social media has become a valuable resource for the study of suicidal ideation and the assessment of suicide risk. Among social media platforms, Reddit has emerged as the most promising one due to its anonymity and its focus on topic-based communities (subreddits) that can be indicative of someone's state of mind or interest regarding mental health disorders such as r/SuicideWatch, r/Anxiety, r/depression. A challenge for previous work on suicide risk assessment has been the small amount of labeled data. We propose an empirical investigation into several classes of weakly-supervised approaches, and show that using pseudo-labeling based on related issues around mental health (e.g., anxiety, depression) helps improve model performance for suicide risk assessment.

==> detailed_table.tex <==
\begin{table*}[]
\centering
\small
% \begin{tabular}{|c|c|c|c|c|c|c|}
\begin{tabular}{|c|c|c|c|c|c|cH|}
\hline
No. & Approach & Setup & a & b & c & d & Macro\\ \hline
1 & Baseline & BERT & 0.742/0.719/0.730 & 0.077/0.077/0.077 & 0.400/0.286/0.333 & 0.525/0.615/0.566 & 0.436/0.424/0.427 \\ \hline
% 0.427/0.712/0.820 \\ \hline %SuicideModel\task_A\BERT\NO_CTL_preprocess_with_no_pretrain\model_neguser5_bert_bsz32_len128_log_2021-01-21_02-53-15_932404
% 2 & XLNET & No & No & No & 0.469/0.723/0.750 & 0.422/0.700/0.828 \\ \hline
% 3 & RoBERTa & No & No & No & 0.463/0.729/0.782 & 0.408/0.731/0.811 \\ \hline
2 & TAP & BERT & 0.774/0.750/0.762 & 0.143/0.154/0.148 & 0.250/0.107/0.150 & 0.588/0.769/0.667 & 0.439/0.445/0.432 \\ \hline
%SuicideModel_backup\task_A\BERT\NO_CTL_preprocess_with_pretrained_sharedtask\model_neguser5_bert_bsz32_gr40_len128_log_2020-12-19_03-57-06_296068
% 0.432/0.740/0.841 \\ \hline
3 & MVL & Word-Mask & 0.788/0.812/0.800 & 0.111/0.077/0.091 & 0.391/0.321/0.353 & 0.567/0.654/0.607 & 0.464/0.466/0.463 \\
% & 0.463 \\
%SuicideRiskPrediction\SuicideModel_aux_word_mask\task_A\BERT\NO_CTL_preprocess_with_no_pretrain\poch20_bsz32_len128\model_epoch20_bsz32_len128_log_2021-01-29_02-00-44_037640
% 0.463/\textbf{0.797}/\textbf{0.865} \\
4 & MVL & Sent-Mask & 0.551/0.844/0.667 & 0.091/0.077/0.083 & 0.294/0.179/0.222 & 0.583/0.538/0.560 & 0.380/0.409/0.383 \\ 
% SuicideRiskPrediction\SuicideModel_aux_sent_mask\task_A\BERT\NO_CTL_preprocess_with_no_pretrain\poch20_bsz32_len128
% & 0.383 \\ 
% 0.383/0.713/0.753 \\ \hline
5 & MVL & BegEd  & 0.686/0.750/0.716 & 0/0/0 & 0.320/0.286/0.302 & 0.531/0.654/0.586 & 0.384/0.422/0.401\\
% & 0.401 \\
% SuicideRiskPrediction\SuicideModel_aux_beged_KL\task_A\BERT\NO_CTL_preprocess_with_no_pretrain\poch20_bsz32_len128\model_epoch20_bsz32_len128_log_2021-01-22_19-10-57_690749
6 & MVL & K-Sum & 0.686/0.750/0.716 & 0/0/0 & 0.320/0.286/0.302 & 0.531/0.654/0.586 & 0.384/0.422/0.401\\
% & 0.401 \\ 
\hline
%SuicideModel_aux_sum_KL\task_A\BERT\NO_CTL_preprocess_with_no_pretrain\poch20_bsz32_len128\model_epoch20_bsz32_len128_log_2021-01-22_19-23-39_430603
% 0.401/0.735/0.806 \\ \hline
7 & PL & \begin{tabular}[c]{@{}c@{}}Depression
\\ (c) 
% \\ 
% (medium-risk)
\end{tabular}  
& 0.913/0.656/0.764 & 0.333/0.231/0.273 & 0.333/0.321/0.327 & 0.561/0.712/0.627 & 0.535/0.480/0.498\\
% & \textbf{0.497} \\
%SuicideRiskPrediction\SuicideModel_backup\task_A\BERT\NO_CTL_preprocess_with_no_pretrain_depopPL\model_neguser5_bert_bsz32_gr40_len128_log_2020-12-22_23-42-26_679490
% \textbf{0.497}/0.728/{0.848} \\ \hline
8 & PL & \begin{tabular}[c]{@{}c@{}}Anxiety\\ 
% (low-risk)
(b)
\end{tabular}  
& 0.808/0.656/0.724 & 0.167/0.154/0.160 & 0.440/0.393/0.415 & 0.565/0.673/0.614 & 0.495/0.469/0.478\\
% & 0.478 \\
%SuicideRiskPrediction\SuicideModel\task_A\BERT\NO_CTL_preprocess_with_no_pretrain_anxiety_b_sample\poch20_bsz32_len128\model_epoch20_bsz32_len128_log_2021-01-25_07-03-07_762352
% 0.478/{0.738}/0.820 \\ \hline
9 & PL & \begin{tabular}[c]{@{}c@{}}Depression \\+ Anxiety
% \\ (low-risk and medium-risk)
\end{tabular}  
& 0.821/0.719/0.767 & 0.133/0.154/0.143 & 0.385/0.357/0.370 & 0.554/0.596/0.574 & 0.473/0.456/0.463 \\
% & 0.463 \\ 

\hline
% SuicideRiskPrediction\SuicideModel\task_A\BERT\NO_CTL_preprocess_with_no_pretrain_depop_anxiety_1_2\poch20_bsz32_len128\model_epoch20_bsz32_len128_log_2021-01-29_20-35-16_722986
% 0.463/0.737/0.846 \\ \hline
10 & PL & \begin{tabular}[c]{@{}c@{}}Task C\\ 
% (low-risk)
(b)
\end{tabular} 
& 0.774/0.750/0.762 & 0.083/0.077/0.080 & 0.438/0.250/0.318 & 0.606/0.769/0.678 & 0.475/0.462/0.460 \\
% & 0.460 \\
%SuicideRiskPrediction\SuicideModel\task_A\BERT\NO_CTL_preprocess_with_no_pretrain_taskC_PL_simp\poch20_bsz32_len128\model_epoch20_bsz32_len128_log_2021-01-22_20-20-54_519436
% 0.460/0.772/0.841 \\ \hline
11 & - & \begin{tabular}[c]{@{}c@{}}Task C\\ (crowd-\\labelled)\end{tabular} 
& 0.760/0.594/0.667 & 0/0/0 & 0.357/0.357/0.357 & 0.556/0.673/0.609 & 0.418/0.406/0.408 \\
% & 0.408 \\ 
%SuicideRiskPrediction\SuicideModel\task_A\BERT\NO_CTL_preprocess_with_no_pretrain_taskC_GT_simp\poch20_bsz32_len128\model_epoch20_bsz32_len128_log_2021-01-22_20-01-49_349968
% 0.408/0.732/0.784 \\ \hline
 \hline
% 9 & BERT & No & No & Sent-Mask & 0.430/0.733/0.777 & 0.383/0.713/0.753 \\ \hline
% 10 & BERT & No & No & BegEd & 0.434/0.714/0.776 & 0.401/0.735/0.806 \\ \hline

\end{tabular}
% 10 & BERT & No & No & BegEd + K-Sum & 0.408/0.742/0.819 & 0.367.0.692/0.775 \\ \hline
% 11 & BERT & No & No & BegEd & 0.434/0.714/0.776 & 0.401/0.735/0.806 \\ \hline
% 12 & BERT & No & No & K-Sum & 0.434/0.714/0.777 & 0.401/0.735/0.806 \\ \hline
% \end{tabular}
\caption{Results Task A test set. %Macro-F1 scores on the test set.
% The performance on both valid set and test set are reported according to the format ``Macro-F1/Urgent-F1/Flagged-F1''. 
% For MVL, due to space limitation, we only present the results of the best two strategies in MVL and more results can be found in Appendix \ref{app: MVL}.
For each of tasks 7-11, the size of added data is 8\% of training data. Metrics are all reported on macro-average. %For all auxiliary data considered in the pseudo-labeling part, we make sure they have the same number of instances, roughly $8\%$ of the training set. 
}
\label{tab:exp-class-decomp-res}
\end{table*}
